A Bayesian Optimization Approach to Machine Translation Reranking

Reranking a list of candidates from a machine translation system with an external scoring model and returning the highest-scoring candidate remains a simple and effective method for improving the overall output quality. Translation scoring models continue to grow in size, with the best models being comparable to generation models. Thus, reranking can add substantial computational cost to the translation pipeline. In this work, we pose reranking as a Bayesian optimization (BayesOpt) problem. By strategically selecting candidates to score based on a balance of exploration and exploitation, we show that it is possible to find top-scoring candidates when scoring only a fraction of the candidate list. For instance, our method achieves the same CometKiwi score using only 70 scoring evaluations compared a baseline system using 180. We present a multi-fidelity setting for BayesOpt, where the candidates are first scored with a cheaper but noisier proxy scoring model, which further improves the cost-performance tradeoff when using smaller but well-trained distilled proxy scorers.

==> meta_model.tex <==
$x_1,...,x_N$ are the candidates (source + target). T is the number of metrics, 
$z_1,...,z_T$ are the metrics that we have.

$\sigma_{z, z'}$ is the covariance between $z$ and $z'$ and can be learned with the training data

$\mathcal{X}=[0,1]^d$ is the domain space

fidelity space $\mathcal{Z}$
\newline
$f(\cdot) = g(z,\cdot)$
\newline
$y = f(x) + \epsilon = g(z_t, x_t) + \epsilon $

$\lambda(z)$ is a known cost of metric $z$
\newline

Input to kernel function is the tuple $(emb(x), z)$, where $emb(x)$ could be the output of the COMET encoder for example.

$\kappa([z, k], [z', x'])=\kappa_0 \sigma_{z,z'}^2 \phi_\mathcal{X}(||x-x'||)$

upper confidence bound (exploration of the candidates)

$\varphi_t(x) = \mu(GP_{t-1}(x)) + \beta^{1/2}_{t} \sigma(GP_{t-1}(x))$


How to select the subset?

$\mathcal{Z}_t(x_t)$ depends on
\begin{enumerate}
    \item $\lambda(z) < \lambda(z_{\bullet})$ which means cost should be lower than highest cost
    \item $\tau_{t-1}(z, x_t) > \gamma(z)$ which means posterior variance should be higher than a threshold - how do we define this threshold (see below)?
    \item we don't want to query in the neighborhood of $z_{\bullet}$ but maybe not necessary for us. 
\end{enumerate}

threshold $\gamma(z) = \kappa_0 \xi(z) \frac{\lambda(z)}{\lambda(z_{\bullet})}^q$ and $\xi$ is the information gain
\begin{itemize}
    \item intuition: how expensive is it and how much information do we get - is it worth it? 
    \item p is the dim of fidelity space $\mathcal{Z}$ and d is the dim of domain space $\mathcal{X}$ and $q=1/(p+d+2)$. Why is d relevant here?
    \item $\kappa_0$ is a constant used in the kernel function
\end{itemize}


\hrule


\paragraph{Internal documents.}
The mtm24-comet-pruning Slack has a limited history, so let's save the links:
\begin{itemize}
    \item GitHub \url{https://github.com/juliusc/efficient_reranking}
    \item Finetuning early exit models
    \begin{itemize}
        \item GitHub Ondra Platek finetuning \url{https://github.com/oplatek/COMET/tree/oplatek-early-exit}
        \item \url{https://wandb.ai/moosenet/efficient_reranking/}
    \end{itemize}
    
    \item Gdoc sheets with results
    \url{https://docs.google.com/spreadsheets/d/1YIMfl9n8rAYh0DzI2Ge_gmaXys2YVjBVyD5B6u5LSvo/}
    \item MTM Wednesday presentation \url{https://docs.google.com/presentation/d/1obVDvEEYqWDanH5CPRb3do4b-TMTny6WEJQZGdE7S28/}
    
\end{itemize}




